Excess Semiannual Variation in Historic Temperature Records

The annual temperature cycle of the earth closely follows the annual cycle of solar flux. At temperate latitudes, both driving and response cycles are well described by a strong annual sinusoidal component and a non-vanishing semiannual component. A new analysis of historical weather station records in the United States determines persistent annual and semiannual variation with high precision. Historical annual temperature ranges are consistent with prior studies. Semiannual temperature cycles were much stronger than expected based on the semiannual solar driving. Instead, these cycles were consistent with multiplicative effects of two annual cycles. Our methods provide a quantitative window into the climate's nonlinear response to solar driving, which is of potential value in testing climate models.

==> ejkiv48n71o.tex <==
\section{Introduction}

Global climate features are often studied through terrestrial averaging of monthly mean temperatures over long periods of time. Several authoritative studies \cite{stine2009changes} \cite{stine2012changes} \cite{mckinnon2013spatial} \cite{legates1990mean} \cite{eliseev2003amplitude} have revealed important global factors and secular trends. Comprehensive weather maps constructed with this data reveal accurate proportionality between the solar flux and the annual variation of temperature, especially at temperate latitudes. Thus, describing the temperature response amounts to stating the relationship between the input and response sine waves. This relationship can be characterized by two quantities: the gain (the magnitude of response, defined as the ratio between temperature and driving amplitudes); and the phase lag (the time delay of response, defined as the difference between temperature and driving cycles) \cite{stine2009changes} \cite{mckinnon2013spatial}. Our analysis of 50 to 130 years of temperature data for 64 weather stations builds strongly on this previously established method. Applying such gain-phase analysis to the semiannual part for mid-latitude stations shows anomalously large semiannual gains, which are not well-explained by linear response theory. Below, we interpret these semiannual amplitudes in terms of nonlinear response.

The gains and phase lags reflect universal factors that are largely consistent throughout the northern hemisphere. It is known that the seasonal albedo, the local absorption of short wave radiation, the re-radiated long wave radiation, and the energy transported elsewhere along prevailing winds and temperature gradients can modulate the net solar flux at any given location \cite{pierrehumbert2010principles}. A significant fraction of the $20$ $\text{GJ/m}^2$ annual variation in solar energy must be absorbed and re-emitted every year. The only accessible reservoir of this magnitude is the oceans, and these have their own well-studied annual temperature cycles \cite{levitus1984annual}. The 
physical mechanism for this global heat transport is time invariant and can thus be probed by a historical analysis of the annual cycles.

==> h5tg93k20to.tex <==
\subsection{LaTeX and Mathematical notation}
\label{sec:latex}
You can also include LaTeX code in your documents. Here is a simple inline equation $e^{i\pi}=-1$ and here's a longer equation, numbered:

\begin{equation}
\label{eqn:some}
\int_0^{+\infty}e^{-x^2}dx=\frac{\sqrt{\pi}}{2}
\end{equation}

==> header.tex <==
% Add any additional LaTeX packages and macros here
\usepackage{siunitx}

%---

\iflatexml
% Add any LateXML specific commands here

%---

\else
% The commands below will only change the exported PDF. Edit or remove as needed

\usepackage{lineno}
\linenumbers

\renewcommand{\sfdefault}{ptm}
\renewcommand{\familydefault}{\sfdefault}


\paperfield{Field of the paper}
\abbrevs{ABC, a black cat; DEF, doesn't ever fret; GHI, goes home immediately.}
\corraddress{Author One PhD, Department, Institution, City, State or Province, Postal Code, Country}
\corremail{correspondingauthor@email.com}
\presentadd{Department, Institution, City, State or Province, Postal Code, Country}
\fundinginfo{Funder One, Funder One Department, Grant/Award Number: 123456, 123457 and 123458; Funder Two, Funder Two Department, Grant/Award Number: 123459}
\fi

%---

==> p64n6m5hfi.tex <==
\twocolumn
